Towards Automated Safety Requirements Derivation Using Agent-based RAG

We study the automated derivation of safety requirements in a self-driving vehicle use case, leveraging LLMs in combination with agent-based retrieval-augmented generation. Conventional approaches that utilise pre-trained LLMs to assist in safety analyses typically lack domain-specific knowledge. Existing RAG approaches address this issue, yet their performance deteriorates when handling complex queries and it becomes increasingly harder to retrieve the most relevant information. This is particularly relevant for safety-relevant applications. In this paper, we propose the use of agent-based RAG to derive safety requirements and show that the retrieved information is more relevant to the queries. We implement an agent-based approach on a document pool of automotive standards and the Apollo case study, as a representative example of an automated driving perception system. Our solution is tested on a data set of safety requirement questions and answers, extracted from the Apollo data. Evaluating a set of selected RAG metrics, we present and discuss advantages of a agent-based approach compared to default RAG methods.

==> sections/4_Methodology.tex <==
% Eventually this is not used

\section{Methodology}
\label{sec:methodology}
\todo[inline]{
\begin{itemize}
    %\item Interpreting the scores
    %\item comparison of the approaches
    \item Introducing modularity and scalability through the use of multiple document agents
    \item Compartmentalising documents into different document agents. 
    \begin{itemize}
        \item Storage for standards based document for compliance checking or definitions
        \item Storage for domain knowledge from previous versions or similar kinds of  usecase
    \end{itemize}
    \item Intermediary knowledge representation - tabular data or technical diagrams converted into text and representation by document agents
    \item Defining task based document agents; different agents accessing different subsets of documents based on the defined subtask 
    %\item Compare and contrast the workflow and contexts of both methods and discuss its effectiveness
\end{itemize}
}
% System prompt: You must use one of the tools provided when answering the user's question. You are a specialized agent designed to answer queries about the part of the document X. You must ALWAYS use at least one of the tools provided when answering a question; do NOT rely on prior knowledge.


% \begin{figure*}
%     \centering
%     \includegraphics[width = \textwidth]{Pics/Architecture_alternative.png}
%     \caption{RAG Pipeline}
%     \label{fig:conventional_rag}
% \end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width = \textwidth]{Pics/Conventional_RAG_Pipeline.png}
    \caption{RAG Pipeline}
    \label{fig:conventional_rag}
\end{figure*}



\textbf{Approach:} 

To incorporate the domain-specific knowledge into the LLMs without the over-head cost of fine-tuning the LLMs for specific tasks, we propose a novel approach that empowers the conventional RAG based approaches to make use of document agents that enables a modular and scalable access to relevant domain-knowledge while serving as a reliable approach to control hallucinations. In addition to the conventional RAG based pipeline showcased in \cite{fig:conventional_rag}



\textbf{Architecture of the Pipeline:}

\textit{Vector Store Index:}
Each document is transformed into the vector representations using the embedding models while still capturing their semantic meaning. The chunks of transformed documents are stored in a Vector Database along with their associated metadata. The vector store compares the query embedding with these stored chunks using a similarity metric to retrieve those chunks that might be relevant to the query. These retrieved chunks are included as context along with the query and processed by the LLM to generate a response.

\textit{Summary Index:} \cite{summaryindex_llamaindex}
It is an iterative, hierarchical method for summarizing the document where a tree-like structure is created with summaries stored at lower levels and summaries in higher levels. This enables handling long complex documents while allowing for storing abstracted information contained in those documents.

\textit{Document Agent} - Paired up a summaryIndex and VectorStore Index for each document. It is shown in \ref{fig:document_agent}
\begin{figure}
    \centering
    \includegraphics[width =0.49\textwidth]{Pics/Document_Agent.png}
    \caption{Document Agent}
    \label{fig:document_agent}
\end{figure}
\textit{Query Engine:}
Retrieves most relevant documents for the query from index, top-k semantic retrieval, 

\textit{Prompt Design Template:} Automated Prompt Engineering Template + Role-based prompting; Introduce Prompt here.

\textit{Embedding Model:}
LLM version
embedding


% \begin{table}[h]
%     \centering
%     \begin{tabular}{|p{3.5cm}|p{3.5cm}|}
%         \hline
%         \textbf{Summary Index} & \textbf{Vector Store Index} \\
%         \hline
%         Provides High-Level Summary of documents & Documents encoded into vectors and stored for supporting semantic similarity enabled searches  \\ \hline
%         Stores key sentences, paragraphs, summaries of documents. & Dense vector embeddings of documents.  \\ \hline
%         Direct keyword based or metadata search & Vector similarity search using cosine similarity or other distance metrics  \\ \hline
%         Ideal for hierarchical navigation and overview task & Ideal for better semantic understanding and fine-grained retrieval  \\ \hline

%     \end{tabular}
%     \caption{A brief comparison between the different types of indices that facilitate Agent based RAG approach.}
%     \label{tab:summary&vectorstoreindex}
% \end{table}
\begin{table}
\caption{A brief comparison between the different types of indices that facilitate Agent based RAG approach.}
\begin{tabularx}{\columnwidth}{@{}XX@{}}
    \toprule
    \textbf{Summary Index} & \textbf{Vector Store Index}\\\midrule
     Provides High-Level Summary of documents & Documents encoded into vectors and stored for supporting semantic similarity enabled searches \\ \midrule
    Stores key sentences, paragraphs, summaries of documents. & Dense vector embedding of documents. \\ \midrule
    Direct keyword based or metadata search & Vector similarity search using cosine similarity or other distance metrics. \\ \midrule
    Ideal for hierarchical navigation and overview task & Ideal for better semantic understanding and fine-grained retrieval. \\\bottomrule
\end{tabularx}
\label{tab:summary&vectorstoreindex}
\end{table}


